When the Abyss Looks Back: Unveiling Evolving Dark Patterns in Cookie Consent Banners

To comply with data protection regulations such as the EU General Data Protection Regulation (GDPR) and the California Consumer Privacy Act (CCPA), websites widely deploy cookie consent banners to collect users' privacy preferences. In practice, however, these interfaces often embed dark patterns that undermine informed and freely given consent. As regulatory scrutiny increases, such patterns have not disappeared but have evolved into subtler and more legally ambiguous forms, making existing detection approaches outdated. We present UMBRA, a consent management platform (CMP)-agnostic system that detects both previously studied patterns (DP1-DP10) and nine newly evolved patterns (DP11-DP19) targeting information disclosure, consent revocation, and legal ambiguity, including pay-to-opt-out schemes, revocation barriers, and fake opt-outs. UMBRA combines text analysis, visual heuristics, interaction tracing, and cookie-state monitoring to capture multi-step consent flows missed by prior tools. We evaluate UMBRA on a manually annotated ground-truth dataset and achieve 99% detection accuracy. We further conduct a large-scale compliance-oriented measurement across 14,000 websites spanning the EU, the US, and top-ranked global domains. Our results show that evolved dark patterns are pervasive: revocation is often obstructed, cookies are set before consent or despite explicit rejection, and opt-out interfaces often fail to prevent third-party tracking. On sites with revocation barriers, cookies increase by 25% on average, and many use insecure attributes that increase exposure to attacks such as XSS and CSRF. Overall, our findings provide evidence of systematic non-compliance and show how evolving consent manipulation erodes user autonomy while amplifying privacy and security risks.

==> table/summary_DP_regulation.tex <==
\begin{comment}
\begin{table}
\centering
\caption{Summary of Dark Pattern Types, Descriptions, and Legal Violations}
\small
\begin{tabular}{>{\bfseries}p{2cm} p{2.5cm} p{3.0cm}}
\toprule
\rowcolor{gray!30}\textbf{Pattern} & \textbf{Description} & \textbf{Regulation} \\
\midrule
DP1 \hspace{3cm} OnlyOptIn & Only Opt-in option on initial Cookie Dialog & GDPR Art. 7(3); EDPB 05/2020: Refusal must be as easy as acceptance \\
\rowcolor{gray!10}
DP2 \hspace{2cm} HighlightedOptIn & Opt-in button highlighted more than Opt-out & GDPR Recital 42, Art. 7(2); EDPB/CNIL: Avoid deceptive design \\
DP3  \hspace{3cm}ObstructWindow & Dialog obstructs the window & GDPR Recital 32, Art. 7(2); EDPB 05/2020: Cookie walls are noncompliant \\
\rowcolor{gray!10}
DP4 \hspace{3cm} ComplexText & Large amount of text on cookie dialog & GDPR Art. 12(1): Information must be clear and accessible \\
DP5 \hspace{3cm} MoreOptions & Multiple layers in cookie dialog & GDPR Art. 7(3); EDPB: Consent withdrawal should not be buried \\
\rowcolor{gray!10}
DP6 \hspace{3cm} AmbiguousClose & Ambiguous Close button in addition to Accept & EDPB 05/2020: Close button not equal to valid consent; CNIL: Intent must match interaction \\
DP7\hspace{3cm}  MultipleDialogs & Multiple distinct cookie dialogs on a page & GDPR Art. 5(1)(a): Multiple dialogs reduce clarity \\
\rowcolor{gray!10}
DP8 \hspace{3cm} PreferenceSlider & At least one slider enabled by default & GDPR Art. 7, Art. 25: Pre-selected options violate freely given consent \\
DP9 \hspace{3cm} CloseMoreCookies & Clicking Close leads to more cookies set & GDPR Art. 6(1)(a); EDPB 05/2020: Passive acceptance is invalid \\
\rowcolor{gray!10}
DP10\hspace{3cm}  OptOutMoreCookies & More cookies set despite clicking Opt-out & GDPR Art. 5(1)(a–f): Tracking after opt-out violates purpose limitation \\
DP11\hspace{3cm}  CookieInfoDisplay & No cookie info on the first page & GDPR Art. 12–13: No transparency on cookie use \\
\rowcolor{gray!10}
DP12 \hspace{3cm} PurposeInfoDisplay & No cookie purpose info on the first page & GDPR Art. 13(1)(c): Purpose must be stated \\
DP13\hspace{3cm}  OptOutPricing & Pricing based on opt-out decision & GDPR Art. 5(1)(b); CCPA §1798.125: Price discrimination must be justified \\
\rowcolor{gray!10}
DP14 \hspace{3cm} ConsentRevocationPossible & Consent revocation not possible & GDPR Art. 7(3); Recital 42: Consent must be withdrawable \\
DP15 \hspace{3cm} RevocationHard & Consent revocation is hard & GDPR Art. 7(3), Recital 42: Revocation must be easy and accessible \\
\rowcolor{gray!10}
DP16 \hspace{3cm} PreConsentCookies & Pre-consent cookie loading & ePrivacy Art. 5(3); CJEU Planet49 (C-673/17); GDPR Recital 32: Consent required before cookies \\
DP17\hspace{3cm}  LegalAmbiguity & Unclear legal basis for cookies & GDPR Art. 6(1), Art. 13(1)(c), Recital 39: Clear lawful basis must be stated \\
\rowcolor{gray!10}
DP18\hspace{3cm}  FakeOptOut & Default rejection is non-functional & GDPR Art. 7(4), Recitals 42–43; EDPB 05/2020: Refusal must be genuine \\
DP19 \hspace{3cm} MultiClickOptOut & Takes more clicks to Opt-in or Opt-out & EDPB Cookie Banner Taskforce (2023); CNIL 2021: Reject must be as easy and visible as Accept \\
\bottomrule
\end{tabular}
\end{table}    
\end{comment}



%\begin{comment}
\begin{table*}[H]
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
%\captionsetup{labelformat=empty}
\caption{Summary of Dark Pattern Types, Descriptions, and Legal Violations}
\label{table:Legal_mappings}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{lll} 
\toprule
\rowcolor[rgb]{0.851,0.851,0.851} \textbf{Pattern}                & \textbf{Description}                         & \textbf{Regulation}                                                                             \\ 
\midrule
DP1  OnlyOptIn                                                    & Only Opt-in option on initial Cookie Dialog  & GDPR Art. 7(3); EDPB 05/2020: Refusal must be as easy as acceptance                             \\
\rowcolor[rgb]{0.949,0.949,0.949} DP2  HighlightedOptIn           & Opt-in button highlighted more than Opt-out  & GDPR Recital 42, Art. 7(2); EDPB/CNIL: Avoid deceptive design                                   \\
DP3  ObstructWindow                                               & Dialog obstructs the window                  & GDPR Recital 32, Art. 7(2); EDPB 05/2020: Cookie walls are noncompliant                         \\
\rowcolor[rgb]{0.949,0.949,0.949} DP4  ComplexText                & Large amount of text on cookie dialog        & GDPR Art. 12(1): Information must be clear and accessible                                       \\
DP5  MoreOptions                                                  & Multiple layers in cookie dialog             & GDPR Art. 7(3); EDPB: Consent withdrawal should not be buried                                   \\
\rowcolor[rgb]{0.949,0.949,0.949} DP6  AmbiguousClose             & Ambiguous Close button in addition to Accept & EDPB 05/2020: Close button not equal to valid consent; CNIL: Intent must match interaction      \\
DP7  MultipleDialogs                                              & Multiple distinct cookie dialogs on a page   & GDPR Art. 5(1)(a): Multiple dialogs reduce clarity                                              \\
\rowcolor[rgb]{0.949,0.949,0.949} DP8  PreferenceSlider           & At least one slider enabled by default       & GDPR Art. 7, Art. 25: Pre-selected options violate freely given consent                         \\
DP9  CloseMoreCookies                                             & Clicking Close leads to more cookies set     & GDPR Art. 6(1)(a); EDPB 05/2020: Passive acceptance is invalid                                  \\
\rowcolor[rgb]{0.949,0.949,0.949} DP10  OptOutMoreCookies         & More cookies set despite clicking Opt-out    & GDPR Art. 5(1)(a–f): Tracking after opt-out violates purpose limitation                         \\
DP11  CookieInfoDisplay                                           & No cookie info on the first page             & GDPR Art. 12–13, Recital 39,58: No transparency on cookie use                                                  \\
\rowcolor[rgb]{0.949,0.949,0.949} DP12  PurposeInfoDisplay        & No cookie purpose info on the first page     & GDPR Art. 13(1)(c), Art. 5(1)(b) : Purpose must be stated                                                      \\
DP13  OptOutPricing                                               & Pricing based on opt-out decision            & GDPR Art. 5(1)(b), Art. 7(4), Recital 42; CCPA §1798.125: Price discrimination must be justified                       \\
\rowcolor[rgb]{0.949,0.949,0.949} DP14  ConsentRevocationPossible & Consent revocation not possible              & GDPR Art. 7(3); Recital 42: Consent must be withdrawable                                        \\
DP15  RevocationHard                                              & Consent revocation is hard                   & GDPR Art. 7(3), Recital 42: Revocation must be easy and accessible                              \\
\rowcolor[rgb]{0.949,0.949,0.949} DP16  PreConsentCookies         & Pre-consent cookie loading                   & ePrivacy Art. 5(1) (a), Art. 7(1), GDPR Recital 30: Consent required before cookies  \\
DP17  LegalAmbiguity                                              & Unclear legal basis for cookies              & GDPR Art. 6(1), Art. 13(1)(c), Recital 39: Clear lawful basis must be stated                    \\
\rowcolor[rgb]{0.949,0.949,0.949} DP18  FakeOptOut                & Default rejection is non-functional          & GDPR Art. 7(4), Recitals 42–43; EDPB 05/2020: Refusal must be genuine.                         \\
DP19  MultiClickOptOut                                            & Takes more clicks to Opt-in or Opt-out       & GDPR Art. 7, Art. 5, Recital 42: Reject must be as easy and visible as Accept    \\
\bottomrule
\end{tabular}
}
\end{table*}

%\end{comment}
